A Formal Framework for Mobile Robot Patrolling in Arbitrary Environments with Adversaries

Using mobile robots for autonomous patrolling of environments to prevent intrusions is a topic of increasing practical relevance. One of the most challenging scientific issues is the problem of finding effective patrolling strategies that, at each time point, determine the next moves of the patrollers in order to maximize some objective function. In the very last years this problem has been addressed in a game theoretical fashion, explicitly considering the presence of an adversarial intruder. The general idea is that of modeling a patrolling situation as a game, played by the patrollers and the intruder, and of studying the equilibria of this game to derive effective patrolling strategies. In this paper we present a game theoretical formal framework for the determination of effective patrolling strategies that extends the previous proposals appeared in the literature, by considering environments with arbitrary topology and arbitrary preferences for the agents. The main original contributions of this paper are the formulation of the patrolling game for generic graph environments, an algorithm for finding a deterministic equilibrium strategy, which is a fixed path through the vertices of the graph, and an algorithm for finding a non-deterministic equilibrium strategy, which is a set of probabilities for moving between adjacent vertices of the graph. Both the algorithms are analytically studied and experimentally validated, to assess their properties and efficiency.

==> pictures/bound.tex <==
\pspicture(0,0)(2,0)

\scriptsize

\newcommand{\node}[2]{\bfseries\shortstack{#1\\$d(\textbf{#1})=#2$}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}_{1}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}

\psmatrix[mnode=circle,colsep=1cm,rowsep=1cm]
\node{01}{4} & \node{02}{2} & \node{03}{4}  \\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}
\biarc{1,1}{1,2}
\biarc{1,2}{1,3}

\endpspicture 

==> pictures/corridor-1.tex <==
\pspicture(0,0)(5,5)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
\target{01}{10}{.05}{.5}	&	\node{02}	&	\node{03}	&	\node{04}\\
			& 			&			& 	\target{05}{6}{.45}{.8}\\
			& 			&			& 	\node{06}\\
\target{10}{10}{.35}{.6}	& 	\node{09}	&	\node{08}	& 	\node{07}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,1}{1,2}
\biarc{1,2}{1,3}
\biarc{1,3}{1,4}

\biarc{1,4}{2,4}
\biarc{2,4}{3,4}
\biarc{3,4}{4,4}

\biarc{4,4}{4,3}
\biarc{4,3}{4,2}
\biarc{4,2}{4,1}

\autoarc{60}{1,1}
\autoarc{0}{1,2}
\autoarc{0}{1,3}
\autoarc{-60}{1,4}

\autoarc{-90}{2,4}
\autoarc{-90}{3,4}
\autoarc{-90}{4,4}

\autoarc{180}{4,3}
\autoarc{180}{4,2}
\autoarc{120}{4,1}


%\nccircle[nodesep=2pt,angle=60]{->}{1,3}{.6cm}
%\nccircle[nodesep=2pt,angle=0]{->}{1,4}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-60]{->}{1,5}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=60]{->}{2,1}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=0]{->}{2,2}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=90]{->}{2,3}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=150]{->}{2,5}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-60]{->}{2,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=0]{->}{2,8}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=90]{->}{3,1}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=90]{->}{3,3}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{3,4}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=90]{->}{3,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{3,7}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{3,8}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=150]{->}{4,1}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{4,2}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=90]{->}{4,3}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{4,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{4,8}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=150]{->}{5,3}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{5,4}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{5,5}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-150]{->}{5,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{5,8}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=150]{->}{6,5}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{6,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{6,7}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-150]{->}{6,8}{.6cm}%_{$\alpha_{1,1}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{1,4}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,4}{1,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,4}{1,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,5}{1,4}%_{$\alpha_{1,3}$}%

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{2,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,5}{2,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,5}{1,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,3}{3,4}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,4}{3,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcanglatexle=-15,border=0.5pt]{3,3}{2,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{3,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{4,1}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{3,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{2,1}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{3,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcanglatexle=-15,border=0.5pt]{3,3}{4,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{3,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{4,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{5,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{2,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,6}{3,6}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{4,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,6}{3,6}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{4,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,6}{5,6}%_{$\alpha_{1,3}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{2,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,8}{3,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{4,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,8}{3,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,8}{4,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,8}{5,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,8}{6,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,8}{5,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{6,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{5,6}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{6,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,5}{5,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,7}{6,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,8}{6,7}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,7}{6,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{6,7}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,5}{6,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{6,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{5,4}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{5,4}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{5,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{5,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{4,2}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,2}{4,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,2}{4,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{4,2}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,2}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,2}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,5}{2,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,6}{2,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{3,7}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,7}{3,6}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,7}{3,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{3,7}%_{$\alpha_{1,3}$}

\endpspicture


==> pictures/corridor.tex <==
\pspicture(0,0)(5,5)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
\target{01}{10}{.05}{.5}	&	\node{02}	&	\node{03}	&	\node{04}\\
			& 			&			& 	\target{05}{6}{.45}{.8}\\
			& 			&			& 	\node{06}\\
\target{10}{10}{.35}{.6}	& 	\node{09}	&	\node{08}	& 	\node{07}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,1}{1,2}
\biarc{1,2}{1,3}
\biarc{1,3}{1,4}

\biarc{1,4}{2,4}
\biarc{2,4}{3,4}
\biarc{3,4}{4,4}

\biarc{4,4}{4,3}
\biarc{4,3}{4,2}
\biarc{4,2}{4,1}

\autoarc{60}{1,1}
\autoarc{0}{1,2}
\autoarc{0}{1,3}
\autoarc{-60}{1,4}

\autoarc{-90}{2,4}
\autoarc{-90}{3,4}
\autoarc{-90}{4,4}

\autoarc{180}{4,3}
\autoarc{180}{4,2}
\autoarc{120}{4,1}


%\nccircle[nodesep=2pt,angle=60]{->}{1,3}{.6cm}
%\nccircle[nodesep=2pt,angle=0]{->}{1,4}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-60]{->}{1,5}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=60]{->}{2,1}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=0]{->}{2,2}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=90]{->}{2,3}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=150]{->}{2,5}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-60]{->}{2,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=0]{->}{2,8}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=90]{->}{3,1}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=90]{->}{3,3}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{3,4}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=90]{->}{3,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{3,7}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{3,8}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=150]{->}{4,1}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{4,2}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=90]{->}{4,3}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{4,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{4,8}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=150]{->}{5,3}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{5,4}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{5,5}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-150]{->}{5,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-90]{->}{5,8}{.6cm}%_{$\alpha_{1,1}$}

%\nccircle[nodesep=2pt,angle=150]{->}{6,5}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{6,6}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=180]{->}{6,7}{.6cm}%_{$\alpha_{1,1}$}
%\nccircle[nodesep=2pt,angle=-150]{->}{6,8}{.6cm}%_{$\alpha_{1,1}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{1,4}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,4}{1,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,4}{1,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,5}{1,4}%_{$\alpha_{1,3}$}%

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{2,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,5}{2,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,5}{1,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,3}{3,4}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,4}{3,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcanglatexle=-15,border=0.5pt]{3,3}{2,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{3,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{4,1}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{3,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{2,1}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{3,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcanglatexle=-15,border=0.5pt]{3,3}{4,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{3,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{4,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{5,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{2,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,6}{3,6}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{4,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,6}{3,6}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{4,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,6}{5,6}%_{$\alpha_{1,3}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{2,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,8}{3,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{4,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,8}{3,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,8}{4,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,8}{5,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,8}{6,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,8}{5,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{6,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{5,6}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{6,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,5}{5,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,7}{6,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,8}{6,7}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,7}{6,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{6,7}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,5}{6,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{6,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{5,4}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,3}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{5,4}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{5,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{5,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{4,2}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,2}{4,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,2}{4,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{4,2}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,2}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,2}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,5}{2,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,6}{2,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{3,7}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,7}{3,6}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,7}{3,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{3,7}%_{$\alpha_{1,3}$}

\endpspicture


==> pictures/domination.tex <==

\pspicture(-2,-12.5)(2,.5)

\begin{scriptsize}

\psset{linewidth=0.5pt,fillstyle=solid,fillcolor=white}

\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](0,0){n0}{\textcolor{white}{\small $06$}}

\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](-1,-1.5){n1}{\textcolor{white}{\small $01$}}
\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](1,-1.5){n2}{\textcolor{white}{\small $11$}}

\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](-1,-3){n3}{\textcolor{white}{\small $02$}}
\cnodeput[linewidth=1pt](1,-3){n4}{\small $12$}
\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](3,-3){n5}{\textcolor{white}{\small $18$}}

\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](-1,-4.5){n6}{\textcolor{white}{\small $03$}}
\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](3,-4.5){n7}{\textcolor{white}{\small $21$}}

\cnodeput[linewidth=1 pt](-1,-6){n8}{\small $07$}
\cnodeput[linewidth=1pt](3,-6){n9}{\small $22$}

\cnodeput[linewidth=1pt](-1,-7.5){n10}{\small $08$}
\cnodeput[linewidth=1pt](3,-7.5){n11}{\small $23$}

\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](-1,-9){n12}{\textcolor{white}{\small $13$}}
\cnodeput[linewidth=1pt](3,-9){n13}{\small $24$}

\cnodeput[linewidth=1pt](-3,-10.5){n14}{\small $14$}
\cnodeput[linewidth=1pt](-1,-10.5){n15}{\small $19$}
\cnodeput[linewidth=1pt](3,-10.5){n16}{\small $19$}

\cnodeput[linewidth=1pt](-1,-12){n17}{\small $24$}
\cnodeput[linewidth=1pt, fillcolor=black, fillstyle=solid](3,-12){n18}{\textcolor{white}{\small $13$}}

\cnodeput[linewidth=1pt](-1,-13.5){n19}{\small $23$}
\cnodeput[linewidth=1pt](3,-13.5){n20}{\small $08$}
\cnodeput[linewidth=1pt](5,-13.5){n21}{\small $14$}


\ncline[linewidth=1pt, fillstyle=solid]{<-}{n0}{n1}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n0}{n2}

\ncline[linewidth=1pt, fillstyle=solid]{<-}{n1}{n3}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n2}{n4}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n2}{n5}

\ncline[linewidth=1pt, fillstyle=solid]{<-}{n3}{n6}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n5}{n7}

\ncline[linewidth=1pt, fillstyle=solid]{<-}{n6}{n8}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n7}{n9}

\ncline[linewidth=1pt, fillstyle=solid]{<-}{n8}{n10}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n9}{n11}

\ncline[linewidth=1pt, fillstyle=solid]{<-}{n10}{n12}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n11}{n13}

\ncline[linewidth=1pt, fillstyle=solid]{<-}{n12}{n14}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n12}{n15}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n13}{n16}

\ncline[linewidth=1pt, fillstyle=solid]{<-}{n15}{n17}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n16}{n18}

\ncline[linewidth=1pt, fillstyle=solid]{<-}{n17}{n19}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n18}{n20}
\ncline[linewidth=1pt, fillstyle=solid]{<-}{n18}{n21}

\end{scriptsize}

\endpspicture

==> pictures/eight-1.tex <==
\pspicture(0,0)(3,15)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
\node{01} & \node{02} & \node{03} & \node{04}\\
\target{05}{8}{.05}{.5} & & & \node{06}\\
\node{07} & & & \node{08}\\
\node{09} & \node{10} & \target{11}{8}{.05}{.3} & \node{12}\\
\node{13} & & & \node{14}\\
\node{15} & & & \target{16}{9}{.45}{.8}\\
\node{17} & \target{18}{8}{.35}{.6} & \node{19} & \node{20}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,1}{1,2}
\biarc{1,2}{1,3}
\biarc{1,3}{1,4}
\biarc{1,4}{2,4}
\biarc{2,4}{3,4}
\biarc{3,4}{4,4}
\biarc{4,4}{5,4}
\biarc{4,4}{4,3}
\biarc{5,4}{6,4}
\biarc{6,4}{7,4}
\biarc{7,4}{7,3}
\biarc{7,3}{7,2}
\biarc{7,2}{7,1}
\biarc{7,1}{6,1}
\biarc{6,1}{5,1}
\biarc{5,1}{4,1}
\biarc{4,1}{4,2}
\biarc{4,1}{3,1}
\biarc{3,1}{2,1}
\biarc{2,1}{1,1}
\biarc{4,2}{4,3}

\autoarc{60}{1,1}
\autoarc{0}{1,2}
\autoarc{0}{1,3}
\autoarc{-60}{1,4}
\autoarc{90}{2,1}
\autoarc{90}{3,1}
\autoarc{90}{4,1}
\autoarc{90}{5,1}
\autoarc{90}{6,1}
\autoarc{120}{7,1}
\autoarc{-90}{2,4}
\autoarc{-90}{3,4}
\autoarc{-90}{4,4}
\autoarc{-90}{5,4}
\autoarc{-90}{6,4}
\autoarc{-120}{7,4}
\autoarc{180}{7,2}
\autoarc{180}{7,3}
\autoarc{180}{4,2}
\autoarc{180}{4,3}


\endpspicture


==> pictures/eight.tex <==
\pspicture(0,0)(3,15)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
\node{01} & \node{02} & \node{03} & \node{04}\\
\target{05}{8}{.05}{.5} & & & \node{06}\\
\node{07} & & & \node{08}\\
\node{09} & \node{10} & \target{11}{8}{.05}{.3} & \node{12}\\
\node{13} & & & \node{14}\\
\node{15} & & & \target{16}{9}{.45}{.8}\\
\node{17} & \target{18}{8}{.35}{.6} & \node{19} & \node{20}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,1}{1,2}
\biarc{1,2}{1,3}
\biarc{1,3}{1,4}
\biarc{1,4}{2,4}
\biarc{2,4}{3,4}
\biarc{3,4}{4,4}
\biarc{4,4}{5,4}
\biarc{4,4}{4,3}
\biarc{5,4}{6,4}
\biarc{6,4}{7,4}
\biarc{7,4}{7,3}
\biarc{7,3}{7,2}
\biarc{7,2}{7,1}
\biarc{7,1}{6,1}
\biarc{6,1}{5,1}
\biarc{5,1}{4,1}
\biarc{4,1}{4,2}
\biarc{4,1}{3,1}
\biarc{3,1}{2,1}
\biarc{2,1}{1,1}
\biarc{4,2}{4,3}

\autoarc{60}{1,1}
\autoarc{0}{1,2}
\autoarc{0}{1,3}
\autoarc{-60}{1,4}
\autoarc{90}{2,1}
\autoarc{90}{3,1}
\autoarc{90}{4,1}
\autoarc{90}{5,1}
\autoarc{90}{6,1}
\autoarc{120}{7,1}
\autoarc{-90}{2,4}
\autoarc{-90}{3,4}
\autoarc{-90}{4,4}
\autoarc{-90}{5,4}
\autoarc{-90}{6,4}
\autoarc{-120}{7,4}
\autoarc{180}{7,2}
\autoarc{180}{7,3}
\autoarc{180}{4,2}
\autoarc{180}{4,3}


\endpspicture


==> pictures/fullyconnected.tex <==
\pspicture(0,-0.5)(0,3.)

\small

% \psmatrix[mnode=circle,colsep=2,rowsep=2]
% 1 & 2\\
% 3 & 4\\
% \endpsmatrix
% \psset{shortput=nab,arrows=->,labelsep=1pt}
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,1}{1,2}_{$\alpha_{1,2}$}
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,1}{2,1}_{$\alpha_{1,3}$}
% 
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{1,1}_{$\alpha_{2,1}$}
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,1}_{$\alpha_{2,3}$}
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,2}_{$\alpha_{2,4}$}
% 
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{1,1}_{$\alpha_{3,1}$}
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{1,2}_{$\alpha_{3,2}$}
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,2}_{$\alpha_{3,4}$}
% 
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{1,2}_{$\alpha_{4,2}$}
% \ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,1}_{$\alpha_{4,3}$}
% 
% \ncangles[nodesep=2pt,angleA=90, angleB=45,armA=.5cm, armB=.95cm, linearc=.25]{1,1}{2,2}_{$\alpha_{1,4}$}
% \ncangles[nodesep=2pt,angleA=-90, angleB=-145, armA=.5cm, armB=.85cm, linearc=.25]{2,2}{1,1}_{$\alpha_{4,1}$}


\psmatrix[mnode=circle,colsep=1.5cm,rowsep=1.85cm]
 & 1 \\
 2 & & 3 \\
\endpsmatrix
\psset{shortput=nab,arrows=->,labelsep=1pt}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,1}_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,3}_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{1,2}_{$\alpha_{2,1}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,3}_{$\alpha_{2,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,2}_{$\alpha_{3,1}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,1}_{$\alpha_{3,2}$}

\nccircle[nodesep=2pt]{->}{1,2}{.3cm}_{$\alpha_{1,1}$}
\nccircle[angle=120,nodesep=2pt]{->}{2,1}{.3cm}_{$\alpha_{2,2}$}
\nccircle[angle=240,nodesep=2pt]{->}{2,3}{.3cm}_{$\alpha_{3,3}$}

\endpspicture

==> pictures/grafo.tex <==
\pspicture(0,-2)(30,9)

\scriptsize

\newcommand{\nodouno}{\bfseries\shortstack{01}}
\newcommand{\nododue}{\bfseries\shortstack{02}}
\newcommand{\nodotre}{\bfseries\shortstack{03}}
\newcommand{\nodosei}{\bfseries\shortstack{06}}
\newcommand{\nodosette}{\bfseries\shortstack{07}}
\newcommand{\nodootto}{\bfseries\shortstack{08}}
\newcommand{\nodoundici}{\bfseries\shortstack{11}}
\newcommand{\nodododici}{\bfseries\shortstack{12}}
\newcommand{\nodotredici}{\bfseries\shortstack{13}}
\newcommand{\nodoquattordici}{\bfseries\shortstack{14}}
\newcommand{\nododiciotto}{\bfseries\shortstack{18}}
\newcommand{\nododiciannove}{\bfseries\shortstack{19}}
\newcommand{\nodoventuno}{\bfseries\shortstack{21}}
\newcommand{\nodoventidue}{\bfseries\shortstack{22}}
\newcommand{\nodoventitre}{\bfseries\shortstack{23}}
\newcommand{\nodoventiquattro}{\bfseries\shortstack{24}}

\psmatrix[mnode=circle,colsep=1.5cm,rowsep=1.5cm]
\nodouno       & \nododue & \nodotre \\
\nodosei         &      & \nodosette & \nodootto      \\
\nodoundici   & \nodododici &      & \nodotredici & \nodoquattordici\\
\nododiciotto &      &      & \nododiciannove\\
\nodoventuno & \nodoventidue & \nodoventitre & \nodoventiquattro\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,1}{1,2}_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{1,1}_{$\alpha_{2,1}$}
\nccircle[nodesep=2pt,angle=60]{->}{1,1}{.3cm}_{$\alpha_{1,1}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{1,3}_{$\alpha_{2,3}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{1,2}_{$\alpha_{3,2}$}
\nccircle[nodesep=2pt,angle=0]{->}{1,2}{.3cm}_{$\alpha_{2,2}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,1}{2,1}_{$\alpha_{1,6}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{1,1}_{$\alpha_{6,1}$}
\nccircle[nodesep=2pt,angle=-60]{->}{1,3}{.3cm}_{$\alpha_{3,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{2,3}_{$\alpha_{3,7}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,3}_{$\alpha_{7,3}$}
\nccircle[nodesep=2pt,angle=150]{->}{2,3}{.3cm}_{$\alpha_{7,7}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{3,2}_{$\alpha_{11,12}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,2}{3,1}_{$\alpha_{12,11}$}
\nccircle[nodesep=2pt,angle=90]{->}{3,1}{.3cm}_{$\alpha_{11,11}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{2,1}_{$\alpha_{11,6}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{3,1}_{$\alpha_{6,11}$}
\nccircle[nodesep=2pt,angle=90]{->}{2,1}{.3cm}_{$\alpha_{6,6}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,1}{4,1}_{$\alpha_{18,21}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{5,1}_{$\alpha_{21,18}$}
\nccircle[nodesep=2pt,angle=150]{->}{5,1}{.3cm}_{$\alpha_{21,21}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,4}{2,4}_{$\alpha_{13,8}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,4}{3,4}_{$\alpha_{8,13}$}
\nccircle[nodesep=2pt,angle=90]{->}{3,4}{.3cm}_{$\alpha_{13,13}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,4}{4,4}_{$\alpha_{13,19}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,4}{3,4}_{$\alpha_{19,13}$}
\nccircle[nodesep=2pt,angle=-90]{->}{4,4}{.3cm}_{$\alpha_{19,19}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{4,4}_{$\alpha_{24,19}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,4}{5,4}_{$\alpha_{19,24}$}
\nccircle[nodesep=2pt,angle=-150]{->}{5,4}{.3cm}_{$\alpha_{24,24}$}


\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{4,1}_{$\alpha_{11,18}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{3,1}_{$\alpha_{18,11}$}
\nccircle[nodesep=2pt,angle=90]{->}{4,1}{.3cm}_{$\alpha_{18,18}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{4,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,8}{3,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,8}{4,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,8}{5,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,8}{6,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,8}{5,8}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{6,4}_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,4}{5,4}_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{6,5}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,5}{5,5}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,7}{6,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,8}{6,7}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,7}{6,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{6,7}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,5}{6,6}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{6,5}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,1}{5,2}_{$\alpha_{21,22}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,2}{5,1}_{$\alpha_{22,21}$}
\nccircle[nodesep=2pt,angle=180]{->}{5,2}{.3cm}_{$\alpha_{22,22}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,2}{5,3}_{$\alpha_{22,23}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{5,2}_{$\alpha_{23,22}$}
\nccircle[nodesep=2pt,angle=180]{->}{5,3}{.3cm}_{$\alpha_{23,23}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{5,4}_{$\alpha_{23,24}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,3}_{$\alpha_{24,23}$}
\nccircle[nodesep=2pt,angle=-90]{->}{3,2}{.3cm}_{$\alpha_{12,12}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{4,2}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,2}{4,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,2}{4,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{4,2}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,2}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,1}%_{$\alpha_{1,3}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,3}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,2}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,4}_{$\alpha_{7,8}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,4}{2,3}_{$\alpha_{8,7}$}
\nccircle[nodesep=2pt,angle=-60]{->}{2,4}{.3cm}_{$\alpha_{8,8}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,4}{3,5}_{$\alpha_{13,14}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,5}{3,4}_{$\alpha_{14,13}$}
\nccircle[nodesep=2pt,angle=-90]{->}{3,5}{.3cm}_{$\alpha_{14,14}$}

%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,7}{3,8}%_{$\alpha_{1,2}$}
%\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{3,7}%_{$\alpha_{1,3}$}


\endpspicture

==> pictures/grafonondominato.tex <==
\pspicture(6,0)(30,12)

\scriptsize

%\newcommand{\nodouno}{\bfseries\shortstack{01\\$d_{01}=1$\\(1,0)}}
%\newcommand{\nododue}{\bfseries\shortstack{02\\$d_{02}=1$\\(1,0)}}
%\newcommand{\nodotre}{\bfseries\shortstack{03\\$d_{03}=1$\\(1,0)}}
%\newcommand{\nodoquattro}{\bfseries\shortstack{04\\$d_{04}=1$\\(1,0)}}
%\newcommand{\nodocinque}{\bfseries\shortstack{05\\$d_{05}=1$\\(1,0)}}
%\newcommand{\nodosei}{\bfseries\shortstack{06\\$d_{06}=7$\\(.2,.6)}}
%\newcommand{\nodosette}{\bfseries\shortstack{07\\$d_{07}=1$\\(1,0)}}
%\newcommand{\nodootto}{\bfseries\shortstack{08\\$d_{08}=7$\\(.3,.8)}}
%\newcommand{\nodonove}{\bfseries\shortstack{09\\$d_{09}=1$\\(1,0)}}
%\newcommand{\nododieci}{\bfseries\shortstack{10\\$d_{10}=1$\\(1,0)}}
%\newcommand{\nodoundici}{\bfseries\shortstack{11\\$d_{11}=1$\\(1,0)}}
%\newcommand{\nodododici}{\bfseries\shortstack{12\\$d_{12}=9$\\(.1,.2)}}
%\newcommand{\nodotredici}{\bfseries\shortstack{13\\$d_{13}=1$\\(1,0)}}
%\newcommand{\nodoquattordici}{\bfseries\shortstack{14\\$d_{14}=9$\\(.2,.7)}}
%\newcommand{\nodoquindici}{\bfseries\shortstack{15\\$d_{15}=1$\\(1,0)}}
%\newcommand{\nodosedici}{\bfseries\shortstack{16\\$d_{16}=1$\\(1,0)}}
%\newcommand{\nododiciassette}{\bfseries\shortstack{17\\$d_{17}=9$\\(1,0)}}
%\newcommand{\nododiciotto}{\bfseries\shortstack{18\\$d_{18}=7$\\(.2,.4)}}
%\newcommand{\nododiciannove}{\bfseries\shortstack{19\\$d_{19}=1$\\(1,0)}}
%\newcommand{\nodoventi}{\bfseries\shortstack{20\\$d_{20}=1$\\(1,0)}}
%\newcommand{\nodoventuno}{\bfseries\shortstack{21\\$d_{21}=1$\\(1,0)}}
%\newcommand{\nodoventidue}{\bfseries\shortstack{22\\$d_{22}=1$\\(1,0)}}
%\newcommand{\nodoventitre}{\bfseries\shortstack{23\\$d_{23}=1$\\(1,0)}}
%\newcommand{\nodoventiquattro}{\bfseries\shortstack{24\\$d_{24}=1$\\(1,0)}}
%\newcommand{\nodoventicinque}{\bfseries\shortstack{25\\$d_{25}=1$\\(1,0)}}
%\newcommand{\nodoventisei}{\bfseries\shortstack{26\\$d_{26}=1$\\(1,0)}}
%\newcommand{\nodoventisette}{\bfseries\shortstack{27\\$d_{27}=1$\\(1,0)}}
%\newcommand{\nodoventiotto}{\bfseries\shortstack{28\\$d_{28}=1$\\(1,0)}}
%\newcommand{\nodoventinove}{\bfseries\shortstack{29\\$d_{29}=1$\\(1,0)}}

\newcommand{\nodouno}{\bfseries\shortstack{\\01\\ ~\hspace{1.05cm}~}}
\newcommand{\nododue}{\bfseries\shortstack{\\02\\ ~\hspace{1.05cm}~}}
\newcommand{\nodotre}{\bfseries\shortstack{\\03\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoquattro}{\bfseries\shortstack{\\04\\ ~\hspace{1.05cm}~}}
\newcommand{\nodocinque}{\bfseries\shortstack{\\05\\ ~\hspace{1.05cm}~}}
\newcommand{\nodosei}{\bfseries\shortstack{06\\$d(06)=9$\\(.1,.6)}}
\newcommand{\nodosette}{\bfseries\shortstack{\\07\\ ~\hspace{1.05cm}~}}
\newcommand{\nodootto}{\bfseries\shortstack{08\\$d(08)=8$\\(.3,.8)}}
\newcommand{\nodonove}{\bfseries\shortstack{\\09\\ ~\hspace{1.05cm}~}}
\newcommand{\nododieci}{\bfseries\shortstack{\\10\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoundici}{\bfseries\shortstack{\\11\\ ~\hspace{1.05cm}~}}
\newcommand{\nodododici}{\bfseries\shortstack{12\\$d(12)=9$\\(.1,.2)}}
\newcommand{\nodotredici}{\bfseries\shortstack{\\13\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoquattordici}{\bfseries\shortstack{14\\$d(14)=9$\\(.2,.7)}}
\newcommand{\nodoquindici}{\bfseries\shortstack{\\15\\ ~\hspace{1.05cm}~}}
\newcommand{\nodosedici}{\bfseries\shortstack{\\16\\ ~\hspace{1.05cm}~}}
\newcommand{\nododiciassette}{\bfseries\shortstack{\\17\\ ~\hspace{1.05cm}~}}
\newcommand{\nododiciotto}{\bfseries\shortstack{18\\$d(18)=8$\\(.3,.6)}}
\newcommand{\nododiciannove}{\bfseries\shortstack{\\19\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventi}{\bfseries\shortstack{\\20\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventuno}{\bfseries\shortstack{\\21\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventidue}{\bfseries\shortstack{\\22\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventitre}{\bfseries\shortstack{\\23\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventiquattro}{\bfseries\shortstack{\\24\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventicinque}{\bfseries\shortstack{\\25\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventisei}{\bfseries\shortstack{\\26\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventisette}{\bfseries\shortstack{\\27\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventiotto}{\bfseries\shortstack{\\28\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventinove}{\bfseries\shortstack{\\29\\ ~\hspace{1.05cm}~}}


\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
      &      & \nodouno & \nododue & \nodotre \\
  &  &  \nodosei &      & \nodosette &  \nodootto      \\
  &      & \nodoundici & \nodododici &      & \nodotredici &  \nodoquattordici  \\
  &  &  \nododiciotto &      &      & \nododiciannove  \\
      &      & \nodoventuno & \nodoventidue & \nodoventitre & \nodoventiquattro \\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}


\nccircle[nodesep=2pt,angle=60]{->}{1,3}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=0]{->}{1,4}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-60]{->}{1,5}{.6cm}%_{$\alpha_{1,1}$}

\nccircle[nodesep=2pt,angle=60]{->}{2,1}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=0]{->}{2,2}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=90]{->}{2,3}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=150]{->}{2,5}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-60]{->}{2,6}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=0]{->}{2,8}{.6cm}%_{$\alpha_{1,1}$}

\nccircle[nodesep=2pt,angle=90]{->}{3,1}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=90]{->}{3,3}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-90]{->}{3,4}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=90]{->}{3,6}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-90]{->}{3,7}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-90]{->}{3,8}{.6cm}%_{$\alpha_{1,1}$}

\nccircle[nodesep=2pt,angle=150]{->}{4,1}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=180]{->}{4,2}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=90]{->}{4,3}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-90]{->}{4,6}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-90]{->}{4,8}{.6cm}%_{$\alpha_{1,1}$}

\nccircle[nodesep=2pt,angle=150]{->}{5,3}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=180]{->}{5,4}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=180]{->}{5,5}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-150]{->}{5,6}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-90]{->}{5,8}{.6cm}%_{$\alpha_{1,1}$}

\nccircle[nodesep=2pt,angle=150]{->}{6,5}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=180]{->}{6,6}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=180]{->}{6,7}{.6cm}%_{$\alpha_{1,1}$}
\nccircle[nodesep=2pt,angle=-150]{->}{6,8}{.6cm}%_{$\alpha_{1,1}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{1,4}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,4}{1,3}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,4}{1,5}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,5}{1,4}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{2,3}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,3}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,5}{2,5}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,5}{1,5}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,3}{3,4}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,4}{3,3}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,3}{2,3}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{3,3}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{4,1}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{3,1}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,1}{2,1}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{3,1}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,3}{4,3}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{3,3}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{4,3}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{5,3}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{2,6}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,6}{3,6}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{4,6}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,6}{3,6}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{4,6}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,6}{5,6}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{2,8}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,8}{3,8}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{4,8}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,8}{3,8}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,8}{4,8}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,8}{5,8}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,8}{6,8}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,8}{5,8}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{6,6}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{5,6}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{6,5}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,5}{5,5}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,7}{6,8}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,8}{6,7}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,7}{6,6}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{6,7}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,5}{6,6}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{6,6}{6,5}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{5,4}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,3}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,5}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{5,4}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{5,6}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{5,5}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,1}{4,2}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,2}{4,1}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,2}{4,3}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{4,2}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,2}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,1}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,3}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,2}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,5}{2,6}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,6}{2,5}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{3,7}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,7}{3,6}%_{$\alpha_{1,3}$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,7}{3,8}%_{$\alpha_{1,2}$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,8}{3,7}%_{$\alpha_{1,3}$}

\endpspicture

==> pictures/graforidotto.tex <==
\pspicture(0,0)(9,9)

\scriptsize

\newcommand{\nodouno}{\bfseries\shortstack{01\\$d(01)=1$\\(1,0)}}
\newcommand{\nododue}{\bfseries\shortstack{02\\$d_{02}=1$\\(1,0)}}
\newcommand{\nodotre}{\bfseries\shortstack{03\\$d_{03}=1$\\(1,0)}}
\newcommand{\nodoquattro}{\bfseries\shortstack{04\\$d_{04}=1$\\(1,0)}}
\newcommand{\nodocinque}{\bfseries\shortstack{05\\$d_{05}=1$\\(1,0)}}
\newcommand{\nodosei}{\bfseries\shortstack{06\\$d(06)=9~$}}
\newcommand{\nodosette}{\bfseries\shortstack{07\\$d_{07}=1$\\(1,0)}}
\newcommand{\nodootto}{\bfseries\shortstack{08\\$d(08)=8~$}}
\newcommand{\nodonove}{\bfseries\shortstack{09\\$d_{09}=1$\\(1,0)}}
\newcommand{\nododieci}{\bfseries\shortstack{10\\$d_{10}=1$\\(1,0)}}
\newcommand{\nodoundici}{\bfseries\shortstack{11\\$d_{11}=1$\\(1,0)}}
\newcommand{\nodododici}{\bfseries\shortstack{12\\$d(12)=9~$}}
\newcommand{\nodotredici}{\bfseries\shortstack{13\\$d_{13}=1$\\(1,0)}}
\newcommand{\nodoquattordici}{\bfseries\shortstack{14\\$d(14)=9~$}}
\newcommand{\nodoquindici}{\bfseries\shortstack{15\\$d_{15}=1$\\(1,0)}}
\newcommand{\nodosedici}{\bfseries\shortstack{16\\$d_{16}=1$\\(1,0)}}
\newcommand{\nododiciassette}{\bfseries\shortstack{17\\$d_{17}=9~$\\(1,0)}}
\newcommand{\nododiciotto}{\bfseries\shortstack{18\\$d(18)=8~$}}
\newcommand{\nododiciannove}{\bfseries\shortstack{19\\$d_{19}=1$\\(1,0)}}
\newcommand{\nodoventi}{\bfseries\shortstack{20\\$d_{20}=1$\\(1,0)}}
\newcommand{\nodoventuno}{\bfseries\shortstack{21\\$d_{21}=1$\\(1,0)}}
\newcommand{\nodoventidue}{\bfseries\shortstack{22\\$d_{22}=1$\\(1,0)}}
\newcommand{\nodoventitre}{\bfseries\shortstack{23\\$d_{23}=1$\\(1,0)}}
\newcommand{\nodoventiquattro}{\bfseries\shortstack{24\\$d_{24}=1$\\(1,0)}}
\newcommand{\nodoventicinque}{\bfseries\shortstack{25\\$d_{25}=1$\\(1,0)}}
\newcommand{\nodoventisei}{\bfseries\shortstack{26\\$d_{26}=1$\\(1,0)}}
\newcommand{\nodoventisette}{\bfseries\shortstack{27\\$d_{27}=1$\\(1,0)}}
\newcommand{\nodoventiotto}{\bfseries\shortstack{28\\$d_{28}=1$\\(1,0)}}
\newcommand{\nodoventinove}{\bfseries\shortstack{29\\$d_{29}=1$\\(1,0)}}

\psmatrix[mnode=circle,colsep=1.75cm,rowsep=1.75cm]
 & \nodosei \\
 \nodododici & \nododiciotto & \nodootto \\
 & \nodoquattordici \\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,1}%_2
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{1,2}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,2}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{1,2}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,3}%_{5}
\ncput*[nrot=0]{5}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,2}%_{5}
\ncput*[nrot=0]{5}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,2}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,1}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,2}%_{7}
\ncput*[nrot=0]{7}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,3}%_{7}
\ncput*[nrot=0]{7}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,2}{2,2}%_{7}
\ncput*[nrot=0]{7}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{3,2}%_{7}
\ncput*[nrot=0]{7}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,2}{2,3}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{3,2}%_{2}
\ncput*[nrot=0]{2}



%\psline[linewidth=3pt,linearc=0.5]{->}(-0,2.5)(0.75,3.25)(-3.75,7.75)(-4.625,7)%(-5.25,6.5)(-3,4.25)

%\psline[linewidth=3pt,linearc=0.5]{->}(-4.625,7)(-5.25,6.25)(-0.75,1.75)(-0,2.5)%(-5.25,6.5)(-3,4.25)


\endpspicture

==> pictures/graforidotto2.tex <==
\pspicture(0,0)(9,9)

\scriptsize

\newcommand{\nodouno}{\bfseries\shortstack{01\\$d_{01}=1$\\(1,0)}}
\newcommand{\nododue}{\bfseries\shortstack{02\\$d_{02}=1$\\(1,0)}}
\newcommand{\nodotre}{\bfseries\shortstack{03\\$d_{03}=1$\\(1,0)}}
\newcommand{\nodoquattro}{\bfseries\shortstack{04\\$d_{04}=1$\\(1,0)}}
\newcommand{\nodocinque}{\bfseries\shortstack{05\\$d_{05}=1$\\(1,0)}}
\newcommand{\nodosei}{\bfseries\shortstack{06\\$d(06)=14$}}
\newcommand{\nodosette}{\bfseries\shortstack{07\\$d_{07}=1$\\(1,0)}}
\newcommand{\nodootto}{\bfseries\shortstack{08\\$d(08)=18$}}
\newcommand{\nodonove}{\bfseries\shortstack{09\\$d_{09}=1$\\(1,0)}}
\newcommand{\nododieci}{\bfseries\shortstack{10\\$d_{10}=1$\\(1,0)}}
\newcommand{\nodoundici}{\bfseries\shortstack{11\\$d_{11}=1$\\(1,0)}}
\newcommand{\nodododici}{\bfseries\shortstack{12\\$d(12)=23$}}
\newcommand{\nodotredici}{\bfseries\shortstack{13\\$d_{13}=1$\\(1,0)}}
\newcommand{\nodoquattordici}{\bfseries\shortstack{14\\$d(14)=22$}}
\newcommand{\nodoquindici}{\bfseries\shortstack{15\\$d_{15}=1$\\(1,0)}}
\newcommand{\nodosedici}{\bfseries\shortstack{16\\$d_{16}=1$\\(1,0)}}
\newcommand{\nododiciassette}{\bfseries\shortstack{17\\$d_{17}=9$\\(1,0)}}
\newcommand{\nododiciotto}{\bfseries\shortstack{18\\$d(18)=18$}}
\newcommand{\nododiciannove}{\bfseries\shortstack{19\\$d_{19}=1$\\(1,0)}}
\newcommand{\nodoventi}{\bfseries\shortstack{20\\$d_{20}=1$\\(1,0)}}
\newcommand{\nodoventuno}{\bfseries\shortstack{21\\$d_{21}=1$\\(1,0)}}
\newcommand{\nodoventidue}{\bfseries\shortstack{22\\$d_{22}=1$\\(1,0)}}
\newcommand{\nodoventitre}{\bfseries\shortstack{23\\$d_{23}=1$\\(1,0)}}
\newcommand{\nodoventiquattro}{\bfseries\shortstack{24\\$d_{24}=1$\\(1,0)}}
\newcommand{\nodoventicinque}{\bfseries\shortstack{25\\$d_{25}=1$\\(1,0)}}
\newcommand{\nodoventisei}{\bfseries\shortstack{26\\$d_{26}=1$\\(1,0)}}
\newcommand{\nodoventisette}{\bfseries\shortstack{27\\$d_{27}=1$\\(1,0)}}
\newcommand{\nodoventiotto}{\bfseries\shortstack{28\\$d_{28}=1$\\(1,0)}}
\newcommand{\nodoventinove}{\bfseries\shortstack{29\\$d_{29}=1$\\(1,0)}}

\psmatrix[mnode=circle,colsep=1.75cm,rowsep=1.75cm]
 & \nodosei \\
 \nodododici & \nododiciotto & \nodootto \\
 & \nodoquattordici \\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,1}%_2
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{1,2}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,2}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{1,2}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,3}%_{5}
\ncput*[nrot=0]{5}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,2}%_{5}
\ncput*[nrot=0]{5}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,2}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,1}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,2}%_{7}
\ncput*[nrot=0]{7}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,3}%_{7}
\ncput*[nrot=0]{7}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,2}{2,2}%_{7}
\ncput*[nrot=0]{7}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{3,2}%_{7}
\ncput*[nrot=0]{7}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,2}{2,3}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{3,2}%_{2}
\ncput*[nrot=0]{2}

\endpspicture

==> pictures/graforidotto3.tex <==
\pspicture(0,0)(9,9)

\scriptsize

\newcommand{\nodouno}{\bfseries\shortstack{01\\$d_{01}=1$\\(1,0)}}
\newcommand{\nododue}{\bfseries\shortstack{02\\$d_{02}=1$\\(1,0)}}
\newcommand{\nodotre}{\bfseries\shortstack{03\\$d_{03}=1$\\(1,0)}}
\newcommand{\nodoquattro}{\bfseries\shortstack{04\\$d_{04}=1$\\(1,0)}}
\newcommand{\nodocinque}{\bfseries\shortstack{05\\$d_{05}=1$\\(1,0)}}
\newcommand{\nodosei}{\bfseries\shortstack{06\\$d(06)=21$}}
\newcommand{\nodosette}{\bfseries\shortstack{07\\$d_{07}=1$\\(1,0)}}
\newcommand{\nodootto}{\bfseries\shortstack{08\\$d(08)=21$}}
\newcommand{\nodonove}{\bfseries\shortstack{09\\$d_{09}=1$\\(1,0)}}
\newcommand{\nododieci}{\bfseries\shortstack{10\\$d_{10}=1$\\(1,0)}}
\newcommand{\nodoundici}{\bfseries\shortstack{11\\$d_{11}=1$\\(1,0)}}
\newcommand{\nodododici}{\bfseries\shortstack{12\\$d(12)=21$}}
\newcommand{\nodotredici}{\bfseries\shortstack{13\\$d_{13}=1$\\(1,0)}}
\newcommand{\nodoquattordici}{\bfseries\shortstack{14\\$d(14)=21$}}
\newcommand{\nodoquindici}{\bfseries\shortstack{15\\$d_{15}=1$\\(1,0)}}
\newcommand{\nodosedici}{\bfseries\shortstack{16\\$d_{16}=1$\\(1,0)}}
\newcommand{\nododiciassette}{\bfseries\shortstack{17\\$d_{17}=9$\\(1,0)}}
\newcommand{\nododiciotto}{\bfseries\shortstack{18\\$d(18)=21$}}
\newcommand{\nododiciannove}{\bfseries\shortstack{19\\$d_{19}=1$\\(1,0)}}
\newcommand{\nodoventi}{\bfseries\shortstack{20\\$d_{20}=1$\\(1,0)}}
\newcommand{\nodoventuno}{\bfseries\shortstack{21\\$d_{21}=1$\\(1,0)}}
\newcommand{\nodoventidue}{\bfseries\shortstack{22\\$d_{22}=1$\\(1,0)}}
\newcommand{\nodoventitre}{\bfseries\shortstack{23\\$d_{23}=1$\\(1,0)}}
\newcommand{\nodoventiquattro}{\bfseries\shortstack{24\\$d_{24}=1$\\(1,0)}}
\newcommand{\nodoventicinque}{\bfseries\shortstack{25\\$d_{25}=1$\\(1,0)}}
\newcommand{\nodoventisei}{\bfseries\shortstack{26\\$d_{26}=1$\\(1,0)}}
\newcommand{\nodoventisette}{\bfseries\shortstack{27\\$d_{27}=1$\\(1,0)}}
\newcommand{\nodoventiotto}{\bfseries\shortstack{28\\$d_{28}=1$\\(1,0)}}
\newcommand{\nodoventinove}{\bfseries\shortstack{29\\$d_{29}=1$\\(1,0)}}

\psmatrix[mnode=circle,colsep=1.75cm,rowsep=1.75cm]
 & \nodosei \\
 \nodododici & \nododiciotto & \nodootto \\
 & \nodoquattordici \\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,1}%_2
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{1,2}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,2}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{1,2}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,2}{2,3}%_{5}
\ncput*[nrot=0]{5}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,2}%_{5}
\ncput*[nrot=0]{5}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,1}{2,2}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,1}%_{2}
\ncput*[nrot=0]{2}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{2,2}%_{7}
\ncput*[nrot=0]{7}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{2,3}%_{7}
\ncput*[nrot=0]{7}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,2}{2,2}%_{7}
\ncput*[nrot=0]{7}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,2}{3,2}%_{7}
\ncput*[nrot=0]{7}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,2}{2,3}%_{2}
\ncput*[nrot=0]{2}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{3,2}%_{2}
\ncput*[nrot=0]{2}

\endpspicture

==> pictures/papero.tex <==
\pspicture(0,0)(4,2)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
\node{01} & \node{02} & \target{03}{6}{.25}{.4} & \node{04} & \node{05}\\
\target{06}{4}{.35}{.5} & & \node{07} & & \node{08}\\
\node{09} & \node{10} & \target{11}{6}{.25}{.4} & \target{12}{5}{.25}{.4} & \node{13}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,1}{1,2}
\biarc{1,2}{1,3}
\biarc{1,3}{1,4}
\biarc{1,4}{1,5}
\biarc{1,1}{2,1}
\biarc{2,5}{1,5}
\biarc{2,5}{3,5}
\biarc{2,1}{3,1}
\biarc{1,3}{2,3}
\biarc{2,3}{3,3}
\biarc{3,1}{3,2}
\biarc{3,2}{3,3}
\biarc{3,3}{3,4}
\biarc{3,4}{3,5}


\endpspicture


==> pictures/ring-1.tex <==
%\pspicture(0,0)(4,5)
\pspicture(0,0)(10,10)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
\target{01}{9}{.05}{.5}		&	\node{02}\\	
\node{15}		& 			&	\node{03}\\
\node{14}		& 			&				& 	\node{04}\\			
\target{13}{9}{.35}{.6}		& 			&				& 			&	\node{05}\\
\node{12}		& 			&				& 			&	\node{06}\\
\node{11}		&	\node{10}	&	\node{09}		&	\node{08}	&	\target{07}{7}{.45}{.8}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,1}{1,2}
\biarc{1,2}{2,3}
\biarc{2,3}{3,4}
\biarc{3,4}{4,5}
\biarc{4,5}{5,5}
\biarc{5,5}{6,5}
\biarc{6,5}{6,4}
\biarc{6,4}{6,3}
\biarc{6,3}{6,2}
\biarc{6,2}{6,1}
\biarc{6,1}{5,1}
\biarc{5,1}{4,1}
\biarc{4,1}{3,1}
\biarc{3,1}{2,1}
\biarc{2,1}{1,1}

\autoarc{60}{1,1}
\autoarc{0}{1,2}
\autoarc{-60}{2,3}
\autoarc{-60}{3,4}
\autoarc{-60}{4,5}
\autoarc{-90}{5,5}
\autoarc{-120}{6,5}
\autoarc{180}{6,4}
\autoarc{180}{6,3}
\autoarc{180}{6,2}
\autoarc{180}{6,1}
\autoarc{90}{5,1}
\autoarc{90}{4,1}
\autoarc{90}{3,1}
\autoarc{90}{2,1}






\endpspicture


==> pictures/ring.tex <==
%\pspicture(0,0)(4,5)
\pspicture(0,0)(10,10)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
\target{01}{9}{.05}{.5}		&	\node{02}\\	
\node{15}		& 			&	\node{03}\\
\node{14}		& 			&				& 	\node{04}\\			
\target{13}{9}{.35}{.6}		& 			&				& 			&	\node{05}\\
\node{12}		& 			&				& 			&	\node{06}\\
\node{11}		&	\node{10}	&	\node{09}		&	\node{08}	&	\target{07}{7}{.45}{.8}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,1}{1,2}
\biarc{1,2}{2,3}
\biarc{2,3}{3,4}
\biarc{3,4}{4,5}
\biarc{4,5}{5,5}
\biarc{5,5}{6,5}
\biarc{6,5}{6,4}
\biarc{6,4}{6,3}
\biarc{6,3}{6,2}
\biarc{6,2}{6,1}
\biarc{6,1}{5,1}
\biarc{5,1}{4,1}
\biarc{4,1}{3,1}
\biarc{3,1}{2,1}
\biarc{2,1}{1,1}

\autoarc{60}{1,1}
\autoarc{0}{1,2}
\autoarc{-60}{2,3}
\autoarc{-60}{3,4}
\autoarc{-60}{4,5}
\autoarc{-90}{5,5}
\autoarc{-120}{6,5}
\autoarc{180}{6,4}
\autoarc{180}{6,3}
\autoarc{180}{6,2}
\autoarc{180}{6,1}
\autoarc{90}{5,1}
\autoarc{90}{4,1}
\autoarc{90}{3,1}
\autoarc{90}{2,1}






\endpspicture


==> pictures/scenario.tex <==
\pspicture(0,0)(6,4.5)

\small

\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(0.3,2.2)(0.3,0.3)(4.4,0.3)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(4.6,0.3)(5.7,0.3)(5.7,1.2)(4.6,1.2)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(4.4,1.2)(3.8,1.2)(3.8,3.3)(4.4,3.3)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(4.6,3.3)(5.7,3.3)(5.7,4.2)(4.6,4.2)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(4.4,4.2)(0.3,4.2)(0.3,2.4)

\psframe[linewidth=0.01](0,0)(1.5,1.5)
\psframe[linewidth=0.01](0,1.5)(1.5,3)
\psframe[linewidth=0.01](0,3)(1.5,4.5)
\psframe[linewidth=0.01](1.5,0)(3,1.5)
\psframe[linewidth=0.01](1.5,2)(3,4.5)
\psframe[linewidth=0.01](3,0)(4.5,1.5)
\psframe[linewidth=0.01](3,1.5)(4.5,3)
\psframe[linewidth=0.01](3,3)(4.5,4.5)
\psframe[linewidth=0.01](4.5,0)(6,1.5)
\psframe[linewidth=0.01](4.5,3)(6,4.5)

\uput[0](0.25,0.6){(1,0)}
\uput[0](1.75,0.6){(1,0)}
\uput[0](3.25,0.6){(1,0)}
\uput[0](4.7,0.6){(.8,.4)}

\uput[0](0.1,2.25){(.7,.5)}
\uput[0](3.25,2.25){(1,0)}

\uput[0](0.25,3.75){(1,0)}
\uput[0](1.75,3.75){(1,0)}
\uput[0](3.25,3.75){(1,0)}
\uput[0](4.7,3.75){(.8,.4)}

\uput[0](0,.2){$d_{07}=1$}
\uput[0](1.5,.2){$d_{08}=1$}
\uput[0](3,.2){$d_{09}=1$}
\uput[0](4.5,.2){$d_{10}=13$}
\uput[0](0.0,1.85){$d_{05}=12$}
\uput[0](3.0,1.85){$d_{06}=1$}
\uput[0](0,3.35){$d_{01}=1$}
\uput[0](1.5,3.35){$d_{02}=1$}
\uput[0](3,3.35){$d_{03}=1$}
\uput[0](4.5,3.35){$d_{04}=14$}

\uput[0](0.4,4.25){\textbf{01}}
\uput[0](1.9,4.25){\textbf{02}}
\uput[0](3.4,4.25){\textbf{03}}
\uput[0](4.9,4.25){\textbf{04}}
\uput[0](0.4,2.75){\textbf{05}}
\uput[0](3.4,2.75){\textbf{06}}
\uput[0](0.4,1.1){\textbf{07}}
\uput[0](1.9,1.1){\textbf{08}}
\uput[0](3.4,1.1){\textbf{09}}
\uput[0](4.9,1.1){\textbf{10}}

\psframe*(1.5,1.5)(3,3)
\psframe*(4.5,1.5)(6,3)


\endpspicture

==> pictures/scenario1.tex <==
\pspicture(0,0)(12,8)

\small

\psframe*[linewidth=0.01](0,0)(1.5,1.5)
\psframe*[linewidth=0.01](0,1.5)(1.5,3)
\psframe[linewidth=0.01](0,3)(1.5,4.5)
\psframe[linewidth=0.01](0,4.5)(1.5,6)
\psframe[linewidth=0.01](0,6)(1.5,7.5)
\psframe*[linewidth=0.01](0,7.5)(1.5,9)

\psframe*[linewidth=0.01](1.5,0)(3,1.5)
\psframe*[linewidth=0.01](1.5,1.5)(3,3)
\psframe[linewidth=0.01](1.5,3)(3,4.5)
\psframe*[linewidth=0.01](1.5,4.5)(3,6)
\psframe[linewidth=0.01](1.5,6)(3,7.5)
\psframe*[linewidth=0.01](1.5,7.5)(3,9)

\psframe*[linewidth=0.01](3,0)(4.5,1.5)
\psframe[linewidth=0.01](3,1.5)(4.5,3)
\psframe[linewidth=0.01](3,3)(4.5,4.5)
\psframe[linewidth=0.01](3,4.5)(4.5,6)
\psframe[linewidth=0.01](3,6)(4.5,7.5)
\psframe[linewidth=0.01](3,7.5)(4.5,9)

\psframe*[linewidth=0.01](4.5,0)(6,1.5)
\psframe[linewidth=0.01](4.5,1.5)(6,3)
\psframe*[linewidth=0.01](4.5,3)(6,4.5)
\psframe[linewidth=0.01](4.5,4.5)(6,6)
\psframe*[linewidth=0.01](4.5,6)(6,7.5)
\psframe[linewidth=0.01](4.5,7.5)(6,9)

\psframe[linewidth=0.01](6,0)(7.5,1.5)
\psframe[linewidth=0.01](6,1.5)(7.5,3)
\psframe*[linewidth=0.01](6,3)(7.5,4.5)
\psframe*[linewidth=0.01](6,4.5)(7.5,6)
\psframe[linewidth=0.01](6,6)(7.5,7.5)
\psframe[linewidth=0.01](6,7.5)(7.5,9)

\psframe[linewidth=0.01](7.5,0)(9,1.5)
\psframe[linewidth=0.01](7.5,1.5)(9,3)
\psframe[linewidth=0.01](7.5,3)(9,4.5)
\psframe[linewidth=0.01](7.5,4.5)(9,6)
\psframe[linewidth=0.01](7.5,6)(9,7.5)
\psframe*[linewidth=0.01](7.5,7.5)(9,9)

\psframe[linewidth=0.01](9,0)(10.5,1.5)
\psframe*[linewidth=0.01](9,1.5)(10.5,3)
\psframe*[linewidth=0.01](9,3)(10.5,4.5)
\psframe[linewidth=0.01](9,4.5)(10.5,6)
\psframe*[linewidth=0.01](9,6)(10.5,7.5)
\psframe*[linewidth=0.01](9,7.5)(10.5,9)

\psframe[linewidth=0.01](10.5,0)(12,1.5)
\psframe[linewidth=0.01](10.5,1.5)(12,3)
\psframe[linewidth=0.01](10.5,3)(12,4.5)
\psframe[linewidth=0.01](10.5,4.5)(12,6)
\psframe[linewidth=0.01](10.5,6)(12,7.5)
\psframe*[linewidth=0.01](10.5,7.5)(12,9)

\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(4.4,2.7)(3.8,2.7)(3.8,4.8)(4.4,4.8)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(4.6,4.8)(5.7,4.8)(5.7,5.7)(4.6,5.7)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(4.4,5.7)(3.8,5.7)(3.8,8.7)(4.4,8.7)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(4.6,8.7)(7.0,8.7)(7.0,7.6)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(7.0,7.4)(7.0,6.3)(8.0,6.3)(8.0,5.7)(8.9,5.7)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{<-}(9.1,4.8)(10.2,4.8)(10.2,5.7)(9.1,5.7)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(8.9,4.8)(8.5,4.8)(8.5,3.8)
\psline[linewidth=2pt,linearc=.25,linecolor=lightgray]{->}(8.5,3.6)(8.5,2.7)(4.6,2.7)

\endpspicture

==> pictures/searchtree.tex <==
\scriptsize

\psset{linewidth=0.5pt,fillstyle=solid,fillcolor=white}

\pspicture(-3,-10)(+3,1)

\cnodeput[linewidth=1pt, fillstyle=solid](0,0){n0}{\small $14$}
\cnodeput[linewidth=1pt, fillstyle=solid](0,-1.5){n1}{\small $08$}
\cnodeput[linewidth=1pt, fillstyle=solid](0,-3){n2}{\small $06$}

%\cnodeput[linewidth=0.5pt, fillstyle=solid](-2,-4.5){n3}{\small $12$}
\cnodeput[linewidth=1pt, fillstyle=solid](0,-4.5){n4}{\small $18$}

%\cnodeput[linewidth=0.5pt, fillstyle=solid](-2,-6){n5}{\small $18$}
%\cnodeput[linewidth=0.5pt, fillstyle=solid](-2,-7.5){n6}{\small $06$}
%\cnodeput[linewidth=0.5pt, fillstyle=solid](-2,-9){n7}{\small $08$}
%\cnodeput[linewidth=0.5pt, fillstyle=solid](-2,-10.5){n8}{\small $14$}

\cnodeput[linewidth=1pt, fillstyle=solid](2,-6){n9}{\small $12$}

\cnodeput[linewidth=0.5pt, fillstyle=solid](2,-7.5){n10}{\small $06$}
\cnodeput[linewidth=0.5pt, fillstyle=solid](2,-9){n11}{\small $08$}
\cnodeput[linewidth=0.5pt, fillstyle=solid](2,-10.5){n12}{\small $14$}

\cnodeput[linewidth=1pt, fillstyle=solid](+4,-7.5){n13}{\small $18$}
\cnodeput[linewidth=1pt, fillstyle=solid](+4,-9){n14}{\small $06$}
\cnodeput[linewidth=1pt, fillstyle=solid](+4,-10.5){n15}{\small $08$}
\cnodeput[linewidth=1pt, fillstyle=solid](+4,-12){n16}{\small $14$}

\cnodeput[linewidth=0.5pt, fillstyle=solid](0,-6){n17}{\small $06$}


\ncline[linewidth=1pt, fillstyle=solid]{->}{n0}{n1} \ncput*{2}
\ncline[linewidth=1pt, fillstyle=solid]{->}{n1}{n2} \ncput*{5}
\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n2}{n3} \ncput*{2}
\ncline[linewidth=1pt, fillstyle=solid]{->}{n2}{n4} \ncput*{2}

\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n3}{n5} \ncput*{2}
\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n5}{n6} \ncput*{2}
\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n6}{n7} \ncput*{5}
\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n7}{n8} \ncput*{2}

\ncline[linewidth=1pt, fillstyle=solid]{->}{n4}{n9} \ncput*{2}
\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n9}{n10} \ncput*{2}
\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n10}{n11} \ncput*{5}
\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n11}{n12} \ncput*{2}

\ncline[linewidth=1pt, fillstyle=solid]{->}{n9}{n13} \ncput*{2}
\ncline[linewidth=1pt, fillstyle=solid]{->}{n13}{n14} \ncput*{2}
\ncline[linewidth=1pt, fillstyle=solid]{->}{n14}{n15} \ncput*{5}
\ncline[linewidth=1pt, fillstyle=solid]{->}{n15}{n16} \ncput*{2}
\ncline[linewidth=0.5pt, fillstyle=solid]{->}{n4}{n17} \ncput*{2}

\uput{0}[280](0.65,.125){\scriptsize$\{08\}$}
\uput{0}[280](0.65,-1.375){\scriptsize$\{06\}$}
\uput{0}[280](.65,-2.875){\scriptsize$\{18\}$}
\uput{0}[280](.82,-4.375){\scriptsize$\{06,12\}$}
%\uput{0}[280](-1.35,-4.375){\scriptsize$\{18\}$}
%\uput{0}[280](-1.35,-5.875){\scriptsize$\{06\}$}
%\uput{0}[280](-1.35,-7.375){\scriptsize$\{08\}$}
%\uput{0}[280](-1.35,-8.875){\scriptsize$\{14\}$}

\uput{0}[280](2.82,-5.875){\scriptsize$\{06,18\}$}
\uput{0}[280](2.65,-7.375){\scriptsize$\{08\}$}
\uput{0}[280](2.65,-8.875){\scriptsize$\{14\}$}

\uput{0}[280](4.65,-7.375){\scriptsize$\{06\}$}
\uput{0}[280](4.65,-8.875){\scriptsize$\{08\}$}
\uput{0}[280](4.65,-10.375){\scriptsize$\{14\}$}

\uput{0}[280](0.55,-5.875){\scriptsize$\{~\}$}

\uput{0}[280](0.65,.125){\scriptsize$\{08\}$}


\uput{0}[280](-0.7,.125){\tiny$1^{\textnormal{st}}$}
\uput{0}[280](-0.7,-1.375){\tiny$2^{\textnormal{nd}}$}
\uput{0}[280](-0.7,-2.875){\tiny$3^{\textnormal{rd}}$}
%\uput{0}[280](-2.7,-4.375){\tiny$4^{\textnormal{th}}$}
%\uput{0}[280](-2.7,-5.875){\tiny$5^{\textnormal{th}}$}
%\uput{0}[280](-2.7,-7.375){\tiny$6^{\textnormal{th}}$}
%\uput{0}[280](-2.7,-8.875){\tiny$7^{\textnormal{th}}$}
%\uput{0}[280](-2.7,-10.375){\tiny$8^{\textnormal{th}}$}
\uput{0}[280](-0.7,-4.375){\tiny$4^{\textnormal{th}}$}
\uput{0}[280](-0.7,-5.875){\tiny$5^{\textnormal{th}}$}
\uput{0}[280](1.3,-5.875){\tiny$6^{\textnormal{th}}$}
\uput{0}[280](1.3,-7.375){\tiny$7^{\textnormal{th}}$}
\uput{0}[280](1.3,-8.875){\tiny$8^{\textnormal{th}}$}
\uput{0}[280](1.3,-10.375){\tiny$9^{\textnormal{th}}$}
\uput{0}[280](3.3,-7.375){\tiny$10^{\textnormal{th}}$}
\uput{0}[280](3.3,-8.875){\tiny$11^{\textnormal{th}}$}
\uput{0}[280](3.3,-10.375){\tiny$12^{\textnormal{th}}$}
\uput{0}[280](3.3,-11.875){\tiny$13^{\textnormal{th}}$}

\endpspicture


==> pictures/strategia.tex <==
\pspicture(6,0)(30,12)

\scriptsize

%\newcommand{\nodouno}{\bfseries\shortstack{01\\$d_{01}=1$\\(1,0)}}
%\newcommand{\nododue}{\bfseries\shortstack{02\\$d_{02}=1$\\(1,0)}}
%\newcommand{\nodotre}{\bfseries\shortstack{03\\$d_{03}=1$\\(1,0)}}
%\newcommand{\nodoquattro}{\bfseries\shortstack{04\\$d_{04}=1$\\(1,0)}}
%\newcommand{\nodocinque}{\bfseries\shortstack{05\\$d_{05}=1$\\(1,0)}}
%\newcommand{\nodosei}{\bfseries\shortstack{06\\$d_{06}=7$\\(.2,.6)}}
%\newcommand{\nodosette}{\bfseries\shortstack{07\\$d_{07}=1$\\(1,0)}}
%\newcommand{\nodootto}{\bfseries\shortstack{08\\$d_{08}=7$\\(.3,.8)}}
%\newcommand{\nodonove}{\bfseries\shortstack{09\\$d_{09}=1$\\(1,0)}}
%\newcommand{\nododieci}{\bfseries\shortstack{10\\$d_{10}=1$\\(1,0)}}
%\newcommand{\nodoundici}{\bfseries\shortstack{11\\$d_{11}=1$\\(1,0)}}
%\newcommand{\nodododici}{\bfseries\shortstack{12\\$d_{12}=9$\\(.1,.2)}}
%\newcommand{\nodotredici}{\bfseries\shortstack{13\\$d_{13}=1$\\(1,0)}}
%\newcommand{\nodoquattordici}{\bfseries\shortstack{14\\$d_{14}=9$\\(.2,.7)}}
%\newcommand{\nodoquindici}{\bfseries\shortstack{15\\$d_{15}=1$\\(1,0)}}
%\newcommand{\nodosedici}{\bfseries\shortstack{16\\$d_{16}=1$\\(1,0)}}
%\newcommand{\nododiciassette}{\bfseries\shortstack{17\\$d_{17}=9$\\(1,0)}}
%\newcommand{\nododiciotto}{\bfseries\shortstack{18\\$d_{18}=7$\\(.2,.4)}}
%\newcommand{\nododiciannove}{\bfseries\shortstack{19\\$d_{19}=1$\\(1,0)}}
%\newcommand{\nodoventi}{\bfseries\shortstack{20\\$d_{20}=1$\\(1,0)}}
%\newcommand{\nodoventuno}{\bfseries\shortstack{21\\$d_{21}=1$\\(1,0)}}
%\newcommand{\nodoventidue}{\bfseries\shortstack{22\\$d_{22}=1$\\(1,0)}}
%\newcommand{\nodoventitre}{\bfseries\shortstack{23\\$d_{23}=1$\\(1,0)}}
%\newcommand{\nodoventiquattro}{\bfseries\shortstack{24\\$d_{24}=1$\\(1,0)}}
%\newcommand{\nodoventicinque}{\bfseries\shortstack{25\\$d_{25}=1$\\(1,0)}}
%\newcommand{\nodoventisei}{\bfseries\shortstack{26\\$d_{26}=1$\\(1,0)}}
%\newcommand{\nodoventisette}{\bfseries\shortstack{27\\$d_{27}=1$\\(1,0)}}
%\newcommand{\nodoventiotto}{\bfseries\shortstack{28\\$d_{28}=1$\\(1,0)}}
%\newcommand{\nodoventinove}{\bfseries\shortstack{29\\$d_{29}=1$\\(1,0)}}

\newcommand{\nodouno}{\bfseries\shortstack{\\01\\ ~\hspace{1.05cm}~}}
\newcommand{\nododue}{\bfseries\shortstack{\\02\\ ~\hspace{1.05cm}~}}
\newcommand{\nodotre}{\bfseries\shortstack{\\03\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoquattro}{\bfseries\shortstack{\\04\\ ~\hspace{1.05cm}~}}
\newcommand{\nodocinque}{\bfseries\shortstack{\\05\\ ~\hspace{1.05cm}~}}
\newcommand{\nodosei}{\bfseries\shortstack{06\\$d(06)=9$\\(.1,.6)}}
\newcommand{\nodosette}{\bfseries\shortstack{\\07\\ ~\hspace{1.05cm}~}}
\newcommand{\nodootto}{\bfseries\shortstack{08\\$d(08)=8$\\(.3,.8)}}
\newcommand{\nodonove}{\bfseries\shortstack{\\09\\ ~\hspace{1.05cm}~}}
\newcommand{\nododieci}{\bfseries\shortstack{\\10\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoundici}{\bfseries\shortstack{\\11\\ ~\hspace{1.05cm}~}}
\newcommand{\nodododici}{\bfseries\shortstack{12\\$d(12)=9$\\(.1,.2)}}
\newcommand{\nodotredici}{\bfseries\shortstack{\\13\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoquattordici}{\bfseries\shortstack{14\\$d(14)=9$\\(.2,.7)}}
\newcommand{\nodoquindici}{\bfseries\shortstack{\\15\\ ~\hspace{1.05cm}~}}
\newcommand{\nodosedici}{\bfseries\shortstack{\\16\\ ~\hspace{1.05cm}~}}
\newcommand{\nododiciassette}{\bfseries\shortstack{\\17\\ ~\hspace{1.05cm}~}}
\newcommand{\nododiciotto}{\bfseries\shortstack{18\\$d(18)=8$\\(.3,.6)}}
\newcommand{\nododiciannove}{\bfseries\shortstack{\\19\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventi}{\bfseries\shortstack{\\20\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventuno}{\bfseries\shortstack{\\21\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventidue}{\bfseries\shortstack{\\22\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventitre}{\bfseries\shortstack{\\23\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventiquattro}{\bfseries\shortstack{\\24\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventicinque}{\bfseries\shortstack{\\25\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventisei}{\bfseries\shortstack{\\26\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventisette}{\bfseries\shortstack{\\27\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventiotto}{\bfseries\shortstack{\\28\\ ~\hspace{1.05cm}~}}
\newcommand{\nodoventinove}{\bfseries\shortstack{\\29\\ ~\hspace{1.05cm}~}}


\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
      &      & \nodouno & \nododue & \nodotre \\
  &  &  \nodosei &      & \nodosette &  \nodootto      \\
  &      & \nodoundici & \nodododici &      & \nodotredici &  \nodoquattordici  \\
  &  &  \nododiciotto &      &      & \nododiciannove  \\
      &      & \nodoventuno & \nodoventidue & \nodoventitre & \nodoventiquattro \\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}


\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{1,4}_{$.4985$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,4}{1,3}_{$.2642$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,4}{1,5}_{$.7358$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,5}{1,4}_{$.1289$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,3}{2,3}_{$.5015$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{1,3}_{$.4182$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{1,5}{2,5}_{$.8711$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,5}{1,5}_{$.0005$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,3}{3,4}_{$.0035$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,4}{3,3}_{$1$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,3}{2,3}_{$.8324$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,3}{3,3}_{$.5818$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,3}{4,3}_{$.1641$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{3,3}_{$.2635$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,3}{5,3}_{$.7365$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{4,3}_{$.6295$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,3}{5,4}_{$.3705$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,3}_{$.0304$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,4}{5,5}_{$.9696$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{5,4}_{$.0785$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,5}{5,6}_{$.9215$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{5,5}_{$.0286$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{5,6}{4,6}_{$.9714$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,6}{5,6}_{$.0870$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{4,6}{3,6}_{$.9130$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{4,6}_{$.0650$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{3,7}_{$.5565$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,7}{3,6}_{$1$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{3,6}{2,6}_{$.3785$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,6}{3,6}_{$.6369$}

\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,5}{2,6}_{$.9995$}
\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{2,6}{2,5}_{$.3631$}



\endpspicture


==> pictures/tree-1.tex <==
\pspicture(0,0)(3,15)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
 & \target{01}{7}{.3}{.5}\\		
 & \node{02}\\
 & \node{03}\\ 
\node{05} & \node{04} & \node{08}\\
\target{07}{7}{.6}{.6} & \target{06}{9}{.7}{.8} & \node{09}\\
 & & \node{10}\\
 & \node{15} & \node{12} & \node{11}\\
 & \target{16}{9}{.6}{.6} & \target{14}{8}{.7}{.8} & \target{13}{8}{.3}{.5}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,2}{2,2}
\biarc{2,2}{3,2}
\biarc{3,2}{4,1}
\biarc{3,2}{4,2}
\biarc{3,2}{4,3}
\biarc{4,1}{5,1}
\biarc{4,2}{5,2}
\biarc{4,3}{5,3}
\biarc{5,3}{6,3}
\biarc{6,3}{7,2}
\biarc{6,3}{7,3}
\biarc{6,3}{7,4}
\biarc{7,2}{8,2}
\biarc{7,3}{8,3}
\biarc{7,4}{8,4}
\autoarc{90}{1,2}
\autoarc{90}{2,2}
\autoarc{70}{3,2}
\autoarc{90}{4,1}
\autoarc{90}{4,2}
\autoarc{-90}{4,3}
\autoarc{90}{5,1}
\autoarc{90}{5,2}
\autoarc{-90}{5,3}
\autoarc{70}{6,3}
\autoarc{90}{7,2}
\autoarc{90}{7,3}
\autoarc{-90}{7,4}
\autoarc{90}{8,2}
\autoarc{90}{8,3}
\autoarc{-90}{8,4}










\endpspicture


==> pictures/tree.tex <==
\pspicture(0,0)(3,15)

\scriptsize

\newcommand{\node}[1]{\bfseries\shortstack{\\#1\\ ~\hspace{1.05cm}~}}
\newcommand{\target}[4]{\bfseries\shortstack{#1\\$d(#1)=#2$\\(#3,#4)}}
\newcommand{\arc}[2]{\ncarc[nodesep=2pt,arcangle=-15,border=0.5pt]{#1}{#2}}
\newcommand{\biarc}[2]{\arc{#1}{#2} \arc{#2}{#1}}
\newcommand{\autoarc}[2]{\nccircle[nodesep=2pt,angle=#1]{->}{#2}{.6cm}}



\psmatrix[mnode=circle,colsep=.7cm,rowsep=.7cm]
 & \target{01}{7}{.3}{.5}\\		
 & \node{02}\\
 & \node{03}\\ 
\node{05} & \node{04} & \node{08}\\
\target{07}{7}{.6}{.6} & \target{06}{9}{.7}{.8} & \node{09}\\
 & & \node{10}\\
 & \node{15} & \node{12} & \node{11}\\
 & \target{16}{9}{.6}{.6} & \target{14}{8}{.7}{.8} & \target{13}{8}{.3}{.5}\\
\endpsmatrix

\psset{shortput=nab,arrows=->,labelsep=1pt}

\biarc{1,2}{2,2}
\biarc{2,2}{3,2}
\biarc{3,2}{4,1}
\biarc{3,2}{4,2}
\biarc{3,2}{4,3}
\biarc{4,1}{5,1}
\biarc{4,2}{5,2}
\biarc{4,3}{5,3}
\biarc{5,3}{6,3}
\biarc{6,3}{7,2}
\biarc{6,3}{7,3}
\biarc{6,3}{7,4}
\biarc{7,2}{8,2}
\biarc{7,3}{8,3}
\biarc{7,4}{8,4}
\autoarc{90}{1,2}
\autoarc{90}{2,2}
\autoarc{70}{3,2}
\autoarc{90}{4,1}
\autoarc{90}{4,2}
\autoarc{-90}{4,3}
\autoarc{90}{5,1}
\autoarc{90}{5,2}
\autoarc{-90}{5,3}
\autoarc{70}{6,3}
\autoarc{90}{7,2}
\autoarc{90}{7,3}
\autoarc{-90}{7,4}
\autoarc{90}{8,2}
\autoarc{90}{8,3}
\autoarc{-90}{8,4}










\endpspicture


==> pictures/trees3.tex <==
\begin{tiny}
% \rotatebox{90}{
\def\dedge{\ncline[linestyle=dashed]}
\psset{radius=1.5pt, dotsize=3pt, linewidth=0.5pt}
\pstree[thislevelsep=0,levelsep=1.5cm]{\Tn} {
    \psset{edge=\ncline}
    \pstree{\TC~[tnpos=a]{patroller}}
    {
        \pstree{\TC*[name=1]\ncput*[nrot=15]{$\textit{move}(01)$}}
        {
            \pstree{\TC*[name=1w]\ncput*[nrot=35]{$\textit{wait}$}}
            {
                \pstree{\TC*[name=1w1]\ncput*[nrot=57]{$\textit{move}(01)$}}{}
                \pstree{\TC*[name=1w2,edge=\dedge]}{}
                \pstree{\TC*[name=1w3,edge=\dedge]}{}
            }
            \Tdot ~{\emph{intruder-}\\\emph{capture}}\ncput*[nrot=50]{$\textit{enter}(01)$}
            \pstree{\TC*[name=12]\ncput*[nrot=-70]{$\textit{enter}(02)$}}
            {
                \pstree{\TC*[name=1w1]\ncput*[nrot=57]{$\textit{move}(01)$}}{}
                \pstree{\TC*[name=1w2,edge=\dedge]}{}
                \pstree{\TC*[name=1w3,edge=\dedge]}{}
            }
            \pstree{\Tdot[name=13] \ncput*{$\ldots$}}{\Tn}
        }
        \pstree{\TC*[name=2]\ncput*[nrot=-50]{$\textit{move}(02)$}}
        {
            \pstree{\TC*[name=2w]\ncput*[nrot=35]{$\textit{wait}$}}
            {
                \pstree{\TC*[name=2w1]\ncput*[nrot=57]{$\textit{move}(01)$}}{}
                \pstree{\TC*[name=2w2,edge=\dedge]}{}
                \pstree{\TC*[name=2w3,edge=\dedge]}{}
            }
            \pstree{\TC*[name=21] \ncput*[nrot=-87]{$\textit{enter}(01)$}}
            {
                \pstree{\TC*[name=2w1]\ncput*[nrot=57]{$\textit{move}(01)$}}{}
                \pstree{\TC*[name=2w2,edge=\dedge]}{}
                \pstree{\TC*[name=2w3,edge=\dedge]}{}
            }
            \Tdot ~{\emph{intruder-}\\\emph{capture}} \ncput*[nrot=-50]{$\textit{enter}(02)$}
            \pstree{\TC*[name=23] \ncput*{$\ldots$}}
            {
\Tn
            }
        }
        \pstree{\TC*[name=3]\ncput*[nrot=-15]{$\textit{move}(06)$}}
        { \Tn \Tn
%            \pstree{\TC*[name=3w] ^{$\mathbf{w}$}}
%            {
%                \pstree{\TC*[name=Aw1,edge=\dedge] ^{1}}{}
%                \pstree{\TC*[name=Aw2,edge=\dedge] ^{2}}{}
%                \pstree{\TC*[name=Aw3,edge=\dedge] _{3}}{}
%            }
%            \pstree{\TC*[name=31] ^{1}}
%            {
%                \Tdot ~{$x^0,y^0_{\r}$} ^{1}
%                \Tdot ~{$x^1,y^1_{\r}$} ^{2}
%                \Tdot ~{$x^1,y^1_{\r}$} _{3}
%            }
%            \pstree{\TC*[name=32] ^{2}}
%            {
%                \Tdot ~{$x^2,y^2_{\r}$} ^{1}
%                \Tdot ~{$x^0,y^0_{\r}$} ^{2}
%                \Tdot ~{$x^2,y^2_{\r}$} _{3}
%            }
%            \Tdot ~{$x^0,y^0_{\r}$} _{3}
        }
    }
}


\ncbox[linearc=.0,boxsize=.0,linestyle=dotted,nodesep=.0]{1}{2}
\naput[nrot=:U, labelsep=0.05]{intruder}
\ncbox[linearc=.0,boxsize=.0,linestyle=dotted,nodesep=.0]{2}{3}
\ncarcbox[linearc=.0,boxsize=.0,linestyle=dotted,arcangle=20,nodesep=.0]{12}{1w}
\ncbox[linearc=.0,boxsize=.0,linestyle=dotted,nodesep=.0]{12}{13}
\naput[nrot=:U, labelsep=0.05]{patroller}
\ncbox[linearc=.0,boxsize=.0,linestyle=dotted,nodesep=.0]{2w}{21}
\naput[nrot=:U, labelsep=0.05]{patroller}
\ncarcbox[linearc=.0,boxsize=.0,linestyle=dotted,arcangle=20,nodesep=.0]{23}{21}
\rput(14.2,4.3){\psframebox*{$\ldots$}}
\rput(5.7,2.8){\psframebox*{$\ldots$}}
\rput(13,2.8){\psframebox*{$\ldots$}}
\rput(0.05,1.25){\psframebox*{$\ldots$}}
\rput(0.90,1.25){\psframebox*{$\ldots$}}
\rput(1.75,1.25){\psframebox*{$\ldots$}}
\rput(3.10,1.25){\psframebox*{$\ldots$}}
\rput(4.00,1.25){\psframebox*{$\ldots$}}
\rput(4.90,1.25){\psframebox*{$\ldots$}}
\rput(6.40,1.25){\psframebox*{$\ldots$}}
\rput(7.30,1.25){\psframebox*{$\ldots$}}
\rput(8.15,1.25){\psframebox*{$\ldots$}}
\rput(9.00,1.25){\psframebox*{$\ldots$}}
\rput(9.85,1.25){\psframebox*{$\ldots$}}
\rput(10.75,1.25){\psframebox*{$\ldots$}}
\end{tiny}

